Improving Aleatoric Uncertainty Quantification in Multi-Annotated Medical Image Segmentation with Normalizing Flows

Quantifying uncertainty in medical image segmentation applications is essential, as it is often connected to vital decision-making. Compelling attempts have been made in quantifying the uncertainty in image segmentation architectures, e.g. to learn a density segmentation model conditioned on the input image. Typical work in this field restricts these learnt densities to be strictly Gaussian. In this paper, we propose to use a more flexible approach by introducing Normalizing Flows (NFs), which enables the learnt densities to be more complex and facilitate more accurate modeling for uncertainty. We prove this hypothesis by adopting the Probabilistic U-Net and augmenting the posterior density with an NF, allowing it to be more expressive. Our qualitative as well as quantitative (GED and IoU) evaluations on the multi-annotated and single-annotated LIDC-IDRI and Kvasir-SEG segmentation datasets, respectively, show a clear improvement. This is mostly apparent in the quantification of aleatoric uncertainty and the increased predictive performance of up to 14 percent. This result strongly indicates that a more flexible density model should be seriously considered in architectures that attempt to capture segmentation ambiguity through density modeling. The benefit of this improved modeling will increase human confidence in annotation and segmentation, and enable eager adoption of the technology in practice.

==> nf.tex <==
\section{Normalizing flows}\label{nf}
% copied from internship paper
A sequence of invertible bijective transformations is referred to as Normalizing Flow (NF) in the modern deep learning research. NFs map a complex distribution $p_{\vect{x}}(\mathrm{X})$ to a more simple distribution $p_{\vect{z}}(\mathrm{Z})$ (normalizing direction) through a chain of transformations. By constraining these transformations to be bijective, an inverse transformations exist that transforms the base distribution $p_0(\vect{z}_0)$ to the complex distribution $p_k(\vect{z}_k)$ (generative direction) and thus, enabling sample generation. In our case, we want to map $p_{\vect{x}}(X)$ from $p_{\vect{z}}(Z)$ and use the NF in its generative direction only and do not use it in the normalizing direction. We optimize a NF with a maximum likelihood objective
% This idea is visualized in Figure \ref{fig:flow}, where $k$ equals the final complex transformed distribution while $i$ denotes the $i$th intermediate distribution of the chain.
\begin{equation}
    \begin{aligned}
        \log p(\mathbf{x})=\log p_{0}\left(\mathbf{z}_{0}\right)-\sum_{i=1}^{K} \log \left|\operatorname{det} \frac{d f_{i}}{d \mathbf{z}_{i-1}}\right|.
    \end{aligned}
    \label{eq:loglikely}
\end{equation}
% \begin{figure}
% \begin{minipage}{1.0\linewidth}
%   \centering
%   \centerline{\includesvg[width=11cm]{images/normalizing-flow}}
% %  \vspace{2.0cm}
%   \caption{Series of consecutive transformations transforming a Gaussian base to a complex non-Gaussian target distribution. Image taken from \textit{Janosh Dev.}~\cite{flowimg}}
%   \label{fig:flow}
% \end{minipage}
% \end{figure}
 As seen in the equation below (Equation \eqref{eq:pflow}) The most simple flow with the ability to contract and expand densities is the planar flow \cite{rezende2016variational}.
\begin{equation}
        g(\vect{x})=\vect{x} + \vect{u}h(\vect{w}^T\vect{x}+\vect{b}).
        \label{eq:pflow}
\end{equation}
The same paper also introduced the radial flow. This flow is comparable to the planar flows in simplicity and therefore experiments have been done with it as well. The radial flow is defined as
\begin{equation}
        g(\vect{x})=\vect{x} + \frac{\beta}{\alpha \left|\vect{x}-\vect{x}_0\right|}(\vect{x}-\vect{x}_0).
\end{equation}



